Learning Lyapunov (Potential) Functions from Counterexamples and Demonstrations

We present a technique for learning control Lyapunov (potential) functions, which are used in turn to synthesize controllers for nonlinear dynamical systems. The learning framework uses a demonstrator that implements a black-box, untrusted strategy presumed to solve the problem of interest, a learner that poses finitely many queries to the demonstrator to infer a candidate function and a verifier that checks whether the current candidate is a valid control Lyapunov function. The overall learning framework is iterative, eliminating a set of candidates on each iteration using the counterexamples discovered by the verifier and the demonstrations over these counterexamples. We prove its convergence using ellipsoidal approximation techniques from convex optimization. We also implement this scheme using nonlinear MPC controllers to serve as demonstrators for a set of state and trajectory stabilization problems for nonlinear dynamical systems. Our approach is able to synthesize relatively simple polynomial control Lyapunov functions, and in that process replace the MPC using a guaranteed and computationally less expensive controller.

==> discussion.tex <==
\section{Discussion}
In this section, we discuss the computational complexity of our method
as well as its completeness. Also, we demonstrate where our framework
stands in formal methods.

\subsection{Computational Complexity}
Now, we discuss the total computational complexity of our method.
Recall that $r$ is the number of unknowns in $V$ and if $V$ is a 
polynomial with maximum degree $\hat{d}$ (for some fixed $\hat{d}$),
then $r$ is polynomial in $n$. For example, if $V$ is quadratic, then
$r = \frac{n(n+1)}{2}$. 
The learner finds an ellipsoid over-approximation
of a half ellipsoid iteratively. 
Using existing analysis on ellipsoid 
methods~\cite{karloff2008linear}, one can show
that the total complexity of the learner (for all
iterations) is 
polynomial in $r$, given fixed values for 
$\Delta$  and $\delta$.

And by Theorem~\ref{thm:termination}, the number
of iteration for finding a robust solution is at most 
$2r^2 \ log(\frac{\sqrt{r}\Delta}{\delta})$, which
is polynomial in $r$. The computational complexity
of the verifier in each iteration is polynomial in 
$n$, for a fixed degree of relaxation $d$. And finally, since in our implementation the MPC
uses an interior-point method, the computational complexity remains
polynomial in $n$ (in each iteration) assuming the 
time horizon $T$ is fixed.

All in all, our method uses different convex optimization
techniques to reduce the complexity
of the control synthesis problem and the overall procedure remains polynomial
in the number of state variables. This theoretically guarantees that our
method can be scaled quite efficiently.

\subsection{Completeness}
Since the computational complexity of our method is polynomial
in the number of state variables, there are several sources of incompleteness. 
Each component has its own incompleteness. First of all, the demonstrator
finds only local optimal solution. To avoid this incompleteness, one can
use Monte Carlo methods with convergence guarantee~\cite{kocsis2006bandit}
to make sure the data generator follows a strategy that stabilizes the system. However, one may argue that Newton-type methods are rich
enough to address trajectory optimization problems.
Another source of incompleteness comes from the verifier. The verifier uses
LMI relaxations with relaxation degree $d$. The precision of the verifier
can be improved by increasing degree of relaxation. However, the 
computational complexity of the verifier is exponential in $d$. And finally,
the last source of incompleteness is the learners concept space which
is restricted to a template polynomial (with degree $\hat{d}$). 
However, using results which
guarantee existence of a polynomial Lyapunov functions~\cite{peet2008polynomial}
(assuming that the system is exponentially stable), 
one can increase $\hat{d}$ and eventually the template
would be rich enough
for the stability property.


\subsection{A Formal Method Perspective}
In the domain of formal methods, our method closes the gap between verification
and synthesis problem. Recall that in the verification problem, we want to develop a procedure
which checks whether a Lyapunov function $V$ with a certain template
exists for a \emph{given} controller. In the synthesis problem, we want
to check whether a \emph{control} Lyapunov function $V$ with a certain
template exists.

The idea of using a demonstrator is based on the fact that designing a 
\emph{probably} correct controller with \emph{huge computational power} 
is easy. However, there are two problems. First, these controllers
demands a lot of resources which makes them impractical; second,
verification of these controllers is practically impossible as the
structure of such controllers can be mathematically complicated.

On one side, we have this easy-to-design and computationally-expensive
controller, which we hard-to-verify \emph{verify}. On the other side, we have
the control \emph{synthesis} problem, which is hard to solve. Our solution
lies between this verification and synthesis problem. 

After termination,
our method either provides a CLF (solves synthesis problem) or
declares no robust Lyapunov function exists for the demonstrator (see Theorem~\ref{thm:syn-ver}). 
In other words, even if there was
a verifier that could verify such complicated controller, failure would have been declared 
as such Lyapunov function does not exists.
Therefore, our procedure either proves no Lyapunov function exists 
(failure in verification) or provides a control Lyapunov function 
(success in synthesis).

As the ultimate goal is to design a controller, one can avoid ``failure
in verification" by providing a demonstrator that respects the Lyapunov function
conditions. In other words, it is sufficient to come up with a demonstrator
for which there are Lyapunov functions (of the form given by the template).
Then, our framework can not terminate with ``failure in verification" and
it is forced to terminate with ``success in synthesis".






==> framework.tex <==
\section{Algorithmic Learning Framework}\label{sec:framework}
As mentioned earlier, finding a control Lyapunov function is a 
computationally expensive problem.
In this section, we introduce a learning framework, to learn a
control Lyapunov function instead of solving for one. 
In other words, our framework learn a proper vector $\vc$ s.t. 
Eq.~\eqref{eq:clf-polynomial} and Eq.~\eqref{eq:clf-safety}.

Our learning framework can be viewed as an \emph{algorithmic
query-based learning}. It is algorithmic, because it provides a formal
guarantee and does not tolerate any error and is query-based, 
because there is a dialogue between the
learner and the teacher(s). Also, it can be viewed as an instance of 
``oracle-guided inductive synthesis"~\cite{jha2015theory}.
In this framework, there are 
two types of queries for learning. The answer to these queries are
generated by two teachers (oracles). One of the teachers is a demonstrator
and the other teacher is a verifier. The presence of the verifier as
the second teacher allows us to provide some formal guarantees and
makes this learning framework algorithmic.

From a high-level point of view, the framework works as follows:
The learner generates a concept given a finite set of observations
(training data). The 
generated concept must conform to the training data provided. Then, it
asks one of the oracles (verifier) if such concept conforms to the 
specification. The verifier either guarantees the the concept is correct or 
gives a counter-example (witness). Then, the learner gives
this witness to the other oracle (demonstrator) and asks for a demonstration
(corresponding to the witness). The counter-example and the
demonstration form an observation and
is added to the training set. Afterwards, the learner generates
a new concept given the new training set. This procedure continues
iteratively and if it terminates a correct concept is generated or the learner
gives up because learning the concept is beyond its ability.


\begin{figure}[!t]
\begin{center}
	\includegraphics[width=0.4\textwidth]{pics/framework}
\end{center}
\caption{Visualization of the learning framework}\label{fig:framework} 
\end{figure}

Formally, the framework $\F(\D, \C, \W, \Phi, \Lea, \Ver, \Dem)$ 
consists of a learner $\Lea$, a verifier oracle $\Ver$ and a demonstrator
oracle $\Dem$. These components are defined over concept space $\C$, 
witnesses space $\W$, demonstration space $\D$ and 
specification $\Phi: \C \rightarrow \bools$. More precisely, 
$\Phi(c): (\forall w \in \W) \ (\exists d \in \D) \ \varphi(c, w, d)$. 
A pair of witness $w$ and demonstration $d$ form an observation 
$o \in \OO: (\W \times \D)$.
The components are
defined as follows (Fig.~\ref{fig:framework}):
\begin{enumerate}
\item $\Lea: 2^\OO \rightarrow (\bools \times \C)$, given a set of observations 
$O \subset \OO$, returns the status of learning 
(fail/pass) and a learned concept $c \in \C$.
\item $\Ver: C \rightarrow (\bools \times \W)$, given a concept $c$,
returns the status of verification (fail/pass) and a counter-example
(witness) $w \in \W$.
\item $\Dem: \W \rightarrow \D$ generates a demonstration $d \in \D$, 
given a witness $w \in \W$.
\end{enumerate}



\begin{algorithm}
	\label{alg:framework}
    \SetAlgoLined
    \KwResult{(success, c)}
    O = $\emptyset$ \;
    \While{true}{
        (success, c) = $\Lea$(O)\;
        \If{$\lnot$success}{
            \Return{(false, c)}\;
        }
        $ $(success, w) = $\Ver$(c)\;
        \If{success}{
            \Return{(true, c)}\;
        }
        O = O $\cup$ {(w, $\Dem$(w))}\;
    }
\caption{Learning Framework}
\end{algorithm}

Formally, the solution is described in Alg.~\ref{alg:framework}.
The procedure is iterative and starts with some initial observation 
(possibly empty). In each iteration, the following
steps are executed: 
\begin{enumerate}[Step 1)]
	\item The learner checks if there exists a concept $c$
that conforms to a finite set of observations $O \subset \OO$, i.e. $(\forall (w, d) \in O) \ \varphi(c, w, d)$
	\begin{enumerate}[(a)]
	\item If no such concept
exists, the learner declares failure ($\Lea(O) = (false, \_)$)
	\item If yes, 
a concept $c \in \C$ is generated ($\Lea(O) = (true, c)$)
	\end{enumerate}
	\item The verifier oracle tests
whether $\Phi(c)$ holds
	\begin{enumerate}[(a)]
	\item If yes ($\Ver(c) = (true, \_)$), the process terminates
successfully ($(true, c)$)
	\item Otherwise, the oracle provides a witness $w \in \W$ s.t. 
$(\not\exists d) \varphi(c, w, d)$ ($\Ver(c) = (false, w)$)
	\end{enumerate}
	\item The demonstrator oracle generates a demonstration $d = \Dem(w)$
	\item Observation $o=(w, d)$ is added to the training set $O$.
\end{enumerate}

Notice that if observations are considered to be witness points 
($\OO = \W$), there would be no need for $\Dem$ and the procedure becomes an 
instance of the counter-example guided inductive synthesis
framework~\cite{solar2006combinatorial,alur2015syntax}.
However, in this article, we distinguish between the witnesses and
the observations used for learning. 

Recall that we wish to find proper values for unknown coefficients
$\vc$ s.t. $(\forall \vx \in X)$ Eq.~\eqref{eq:clf-polynomial} and
Eq.~\eqref{eq:clf-safety} hold. Informally speaking, the idea is to
learn CLF from demonstration or
in other words, the CLF is learned using controller
input/output ($\vx$/$\vu$) examples. For this purpose, we define
the observation as $X \times U$. 

As a result, by reformulating the specification we wish to find a $\vc$ s.t. 
$(\forall \vx \in X) \ (\exists \vu \in U)$
\begin{equation}\label{eq:main-constraints}
	\begin{array}{rl}
	(\vx = \vzero) \implies & V(\vx) = 0 \\
	(\vx \in S \setminus \vzero) \implies & V_\vc(\vx) > 0 \\
	(\vx \in S \setminus \vzero) \implies & \nabla V_\vc(\vx).f(\vx, \vu) < 0 \\
	(\vx \in \partial S) \implies & V_\vc(\vx) > \beta \\
	(\vx \in I) \implies & V_\vc(\vx) < \beta 
	\end{array}
\end{equation}

And to instantiate the learning framework,
we consider $C$ to be the concept space $\C$, $X$ to be the witness
space $\W$ and $U$ to be the demonstration space $\D$. Consequently, $\varphi(c, w, d)$ becomes Eq.~\eqref{eq:main-constraints}. Now, we 
state what is formally guaranteed when we use
Alg.~\ref{alg:framework}.

\begin{theorem} \label{thm:syn-ver}
	Alg.~\ref{alg:framework} terminates with two
	possible outcomes: Either there exists a
	control Lyapunov function or, it can be proved
	that ``no Lyapunov function of the specified form
	(Eq.~\eqref{eq:clf-template}) exists for proving
	stability of the demonstrator".
\end{theorem}

Having the big picture of the framework, in the rest of this article, we
discuss the components and their implementations in details.


==> learner.tex <==
\section{Implementing the Learner}
Recall that the learner needs to check if there exists a $\vc$ that respects 
the specification for the training data. In other words, we wish to check
$(\exists \vc \in \C) \ (\forall (\vx, \vu) \in O)$ Eq.~\ref{eq:main-constraints}.
Each observation $(\vx, \vu)$ should satisfy 
Eq.~\ref{eq:main-constraints}. On the other hand, by definition 
(Eq.~\eqref{eq:clf-template}) $V_\vc$ and $\nabla V_\vc.f$ are linear in $\vc$.
Each observation $(\vx, \vu)$ enforces at least one linear 
condition, i.e. $\va . \vc < b$ for some $\va \in \reals^r$ and $b \in \reals$.
Therefore, having a train set, one can use linear programming to check wether
a feasible concept exists.

Also, the learner should provide a concept. For that purpose, we consider the
learner within the framework (instead of considering it isolated) to study the
behavior of the whole framework, assuming that the oracles are provided.
It makes sense to use the linear
programming to find a feasible concept as well:
Assume $P_i$ is the set of feasible concepts in the $i^{th}$ iteration
and $\vc_i \in P_i$ is the learned concept for that iteration. Then, if
there is a counter-example $\vx_i$, there would be a new observation $(\vx_i, \vu_i)$ in
the next iteration.
Since $\vx_i$ is a counter-example 
($(\not\exists \vu \in U) \varphi(\vc_i, \vx_i, \vu)$),
$\vc_i$ does not satisfy $\varphi(\vc_i, \vx_i, \vu_i)$. As a result,
there would be at least one linear constraint 
$H_{i+1} = \{\va . \vc < b \}$ s.t.
$\vc_i \not\in H_{i+1}$. In the next iteration, $\vc_{i+1}$ will not 
remain in the set of feasible concepts as $P_{i+1} \subseteq P_{i} \cap H_{i+1}$.
Hence, the set of feasible sets gets smaller and smaller in each
iteration until it gets empty.

Implementing this procedure is effective as there are efficient solutions
for solving linear programming.
In fact, our main motivation for using demonstration and proposing such
framework is the ability to generate a concept effectively.


So far it is discussed that the learner can be implemented
very efficiently. However, we are interested in proving the termination
of the procedure. More precisely,
we wish to provide another technique for generating a candidate concept
which guarantees termination, as the procedure 
described so far does not guarantee termination.

Alternative to teaching, where the teacher wants to
teach with optimal number of examples, we wish to push the burden of optimal
learning to the learner. In other words, we wish the learner to choose wisely 
in order to experience as few number of failures as possible. Alternative
to teaching dimensions~\cite{goldman1995complexity}, we introduce mislearning
dimensions.

Previous efforts characterize the teaching dimension in discrete
domains~\cite{goldman1995complexity}, where the goal is the exact identification
of a target concept. Corresponding to that, we need some notion of robustness
to deal with the continuous domain. 

\begin{definition}[Robust Correct Concept] A concept $\vc$ is 
$\delta$-correct if $(\forall \hat{\vc} \in B_\delta(\vc))$, $\Phi(\hat{\vc})$,
where $B_\delta(\vc)$ is a $r$-ball centered at $\vc$ with radius $\delta$.
\end{definition}

We assume all parameters (to be learned) belong to 
$[-\Delta, \Delta]^r$ and a $\delta$-correct
concept exists for fixed $\Delta$ and $\delta$.


\begin{definition}[Mislearning dimension] When the learner guesses a wrong concept
, the teacher provides a new observation (example) to refute
the proposed concept. Given a concept class $\C$, the mislearning dimension ($MD$) is 
the minimum number of wrong concepts that the learner can suggest before identifying
a correct concept, having an arbitrary consistence teacher.
\end{definition}

The idea is that a smart student provides a guess, which is very different 
from previous guesses. By using each guess,
a smart learner tries to explore different aspects of the learning concept.
The hope is to achieve a solution within a few iterations. 
Ultimately, we wish the learning framework to terminate in $MD + 1$
iterations. We provide an over-approximation of $MD$ ($\hat{MD}$), which is
polynomial in $r$. Our solution is constructive and we can provide a
procedure which is guaranteed to terminates in $\hat{MD} + 1$ iterations.

Our method either provides a solution or guarantees that no $\delta$-robust
solution exists. The method is simple and is inspired by ellipsoid methods
for convex optimization.
In the $i^{th}$ iteration, the learner 
keeps an ellipsoid $\E_i$, which contains the feasible concepts 
($\E_i \supset P_i$). Hence, $\E_0 = B_{\sqrt{r}\Delta}$.

At each iteration, the learner provides center of $\E_i$ ($\Cen(\E_i)$) as
the guess. For now, assume that $\Cen(\E_i)$ is feasible 
($\Cen(\E_i) \in P_i$). Then, the teachers provide an observation that 
refute $\Cen(\E_i)$ and there is at least one linear constraint 
$H = \{\va. \vc \leq b\}$ s.t. $\va . \Cen(\E_i) = b^* > b$.
Then $H^* = \{\va . \vc \leq b^*\}$ is a hyper-plane that crosses the center
of $\E_i$ and divide it in half (see Fig.~\ref{fig:ellipsoid}). It is 
clear that $\E_i \cap H^*$ over-approximates the feasible concepts.
Similar to ellipsoid method, the 
learner calculates an ellipsoid $\E_{i+1}$ that contains $\E_i \cap H^*$
and as a result, over-approximates the feasible concepts.
This procedure goes on until the volume of the ellipsoid drops
below a threshold. 

\begin{figure}[!t]
\begin{center}
	\includegraphics[width=0.25\textwidth]{pics/ellipsoid}
\end{center}
\caption{Ellipsoids and Generating Candidate Concepts}\label{fig:ellipsoid} 
\end{figure}


Recall that we have assumed $\Cen(\E_i) \in P_i$. In case 
$\Cen(\E_i) \not\in P_i$, the learner does not need more observation
to refute $\Cen(\E_i)$. In fact, the learner can use all the observations 
to performs several iterations within $i^{th}$ iteration until it finds
a feasible guess. More precisely, 
the $\Lea$ will be defined as described in Alg.~\ref{alg:ellipsoid}.

\begin{algorithm}
	\label{alg:ellipsoid}
    \SetAlgoLined
    \SetKwInput{Initialization}{Initialisation}
    \SetKwProg{Fn}{Function}{}{}
    \SetKwRepeat{Do}{do}{while}
    \KwResult{(success, c)}
    \Initialization{$\E$ = $B_{\sqrt{r}\Delta}$}
    \Fn{$\Lea$(O)}{
        $\scr{P}$ := generate feasible polytope from O \;
        \If{$\scr{P}$ = $\emptyset$}{
            \Return{(false, \_)}\;
        }
        \Do{$\Cen$($\E$) $\not\in \scr{P}$}{
	        extract H = \{a.c $<$ b\} from O s.t. a.$\Cen$($\E$) $\geq$ b \;
    	    H$^*$ := \{a.c $<$ a.$\Cen(\E)$\} \;
        	$\E$ := Ellipsoid($\E$, H$^*$) \;
        }
        \Return{($\Vol$($\E$) $\geq$ $B_\delta$, $\Cen$($\E$))}\;
    }
\caption{Ellipsoid Method for the Learner}
\end{algorithm}

Now, we show that there is an upper-bound ($\hat{MD}$) on the 
number of iterations and if there exists a robust correct
concept, the learner finds it in $\hat{MD} + 1$ iterations.

\begin{theorem}\label{thm:termination}
	Given two oracles and $\Lea$ defined in Alg.~\eqref{alg:ellipsoid}, 
	the learning procedure terminates in less than 
	$\hat{MD} + 1t = 2r^2 \ log(\frac{\Delta}{\delta})$ iterations.
\end{theorem}
\begin{proof}
	Using results from geometry of ellipsoids~\cite{karloff2008linear}, the following holds 
\begin{equation}\label{eq:ellipsoid-volume}
\Vol(\E') < e^\frac{-1}{2r} \Vol(\E) \,,
\end{equation}	
where $\E$ and $\E'$ are $\E$ in the RHS and LHS of Line 8 of 
Alg.~\ref{alg:ellipsoid}. Therefore,
\begin{equation}
	\Vol(\E_{i+1}) < e^\frac{-1}{2r} \Vol(\E_i) \,.
\end{equation}
	In addition, $\Vol(\E_0) = \beta_r (\sqrt{r}\Delta)^r$, where $\beta_r$ is
	the volume of
	unit ball in $\reals^r$. Now, suppose that the procedure
	does not terminate in $K = 2r^2 \ log(\frac{\sqrt{r}\Delta}{\delta})$ 
	iterations. Then
	\begin{align*}
		\Vol(\E_K) & < \Vol(\E_0) (e^\frac{-1}{2r})^K \\
		& = \beta_r (\sqrt{r}\Delta)^r (e^\frac{-2r^2 \ log(\frac{\sqrt{r}\Delta}{\delta})}{2r}) \\
		& = \beta_r (\sqrt{r}\Delta)^r (\frac{\delta}{\sqrt{r}\Delta})^r = \beta_r \delta^r = B_\delta
	\end{align*}
	
	However, procedure terminates within first $K$ iterations 
	if $\Vol(\E_K) < B_\delta$, which is a contradiction.
\end{proof}



==> oracles.tex <==
\section{Implementing the Oracles}\label{sec:imp}

So far, we assumed that the oracles are give. In this section, we explain
each oracle in detail and how they can be implemented using
off-the-shelf methods. First, different methods for demonstration is discussed.
And after that, the verifier oracle is investigated.

\subsection{Demonstration}

The demonstrator has a very simple interface: given a state
$\vx$, provide a proper input $\vu$ for that state. Looking from a theoretical
perspective, this oracle can provide (numerical) solutions and one
may complain that if he/she could solve such problem, then there would
be no need for the learning framework.

First, generating demonstrations can be a computationally
demanding procedure. In this framework, the demonstrator is used offline with
much more computational resources. This is more
appealing for problems with time constraints like robotics and embedded
systems. And second, using the proposed 
learning framework, one can find a symbolic solution (value function) and 
having a symbolic solution, verification of the system becomes possible.

Here we provide some possible implementations for this oracle:

\paragraph{Expert:} An expert can use a thought process involving
experiments and reasoning to come up with a solution. The expert can be a
human being. An expert with a lot of experience does not know the exact
policy symbolically, but can provide proper feedback based on his/her
knowledge. Also, the expert generates the data offline and he/she has
much more time for his/her decision and the error rate will reduces
significantly. Also, there would be no need for human resources at
runtime once a controller is learned.

\paragraph{Sample Based Randomized Algorithms:} Sample based algorithms
have been widely investigated using PRM~\cite{kavraki1996probabilistic},
RRTs~\cite{lavalle2000rapidly} and bandit-based planning~\cite{kocsis2006bandit}.
In these methods, a feasible open-look
trajectory from an initial state to a goal state is generated by sampling.
Therefore, these methods are suitable to be used as a demonstrator.
Also, the sampling can happen offline and as a result, they can give a
near-optimal solution with high probability.

\paragraph{Offline Trajectory Optimization:} 
Any offline trajectory optimization 
techniques cover a wide range of techniques
including techniques from optimal control 
(e.g. DDP~\cite{jacobson1970differential}, iLQR~\cite{li2004iterative})
and model predictive control~\cite{camacho2013model} (MPC).
MPC is shown to be
very successful for many problems. Nevertheless, one of the main shortcomings
is the fact that MPC needs a lot of computational power. 
Some of MPC methods try to solve MPC
problems by finding a global optimum~\cite{raff2006nonlinear,franze2009off},
while most of these methods concede to a local optimum and use a Newton-type 
optimization~\cite{diehl2009efficient}. However, if
these methods stop prematurely, the solution would not be optimal
or even feasible, leading to catastrophic results. Using these
methods allows us to get good
solutions for many cases as the demonstrator is used offline and
the computational resources can be provided.


\paragraph{Our Implementation:} In this article, we use offline MPC to
implement the demonstrator. In fact, to demonstrate that offline MPC
can be implemented really easily, we will use a very simple formulation
for the problem and use a general solver to find a solution: first, given
the plant model, the time is discretized with step-size $\tau$ and time
horizon $T$. Then, the goal is to find input sequence 
$\vu(0),\ldots, \vu(T)$ that minimizes the cost function
\begin{align*}
&J(\vx,\vu(0),\ldots,\vu(T)) \\ 
&= \left(\sum_t Cost(\vx(t), \vu(t))\right)
+ TCost(x(T))\\ 
\mbox{s.t. } & \vx(0) = \vx \,, (\forall t) \ \vu(t) \in U \\
&(\forall t > 0) \ \vx(t) = F(\vx(t-\tau), \vu(t-\tau)) \,,
\end{align*}

where $F$ describes the discretized dynamics, $Cost$ is the operation 
cost and $TCost$ is a terminal cost function. Also, for finding
a solution, we use MATLAB's \emph{fmincon} function configured to use
interior-point method algorithm.

\subsection{Verification}
The second oracle is responsible for testing. The oracle should either verify
that the guessed $V$ is a CLF or provide a counter-example $\vx^*$. This oracle
in computer science is generally implemented using SMT solvers. For a given
$\vc$, the oracle needs to check if $(\exists \vx^*) \ \lnot \varphi(\vc, \vx^*)$. 
As mentioned before, $\varphi$ is Eq.~\eqref{eq:clf-polynomial} $\land$ 
Eq.~\eqref{eq:clf-safety}. The hardest part of this problem is the
quantifier alternation in the third condition for Eq.~\eqref{eq:clf-polynomial}:
\[
(\forall \vx \in S \setminus \vzero) \ (\exists \vu \in U) \ \nabla V_\vc.f(\vx, \vu) < 0 \,.
\]
To avoid such an expensive procedure, we use theory of separating hyper-planes
to replace $\exists \vu$ with $\forall \lambda$. Recall that,
$U$ is a polytope defined as $U = \{\vu | A \vu \leq \vb \}$, where
$A \in \reals^{l \times m}$ and $\vb \in \reals^l$. Also, since
$\nabla V_\vc.f(\vx, \vu) = \nabla V_\vc.(f(\vx) + g(\vx)\vu)$ is affine
in $\vu$, $(\exists \vu \in U) \ \nabla V_\vc.f(\vx, \vu) < 0$ can be
replaced by the following:
\[
\begin{array}{ll}
	(\forall \vlam \in \reals^{+l}) & \\
	& A^T \vlam = (\nabla V_\vc.g(\vx))^T \\
	& \vb^T.\vlam \geq -\nabla V_\vc.f(\vx) \,.
\end{array}
\]

Using this trick, $\lnot \varphi(\vc, \vx)$ will have the following form:
\begin{equation}\label{eq:varphi-simple}
\begin{array}{cc}
	& V_\vc(\vzero) =  0  \\
	(\forall \vx \in S \setminus \vzero)& \  V_\vc(\vx) > 0  \\
	(\forall \vx \in \partial S)& \ V_\vc(\vx) > \beta  \\
	(\forall \vx \in I)& \ V_\vc(\vx) < \beta \\
	(\forall \vx \in S \setminus \vzero, \vlam \in \reals^{+l})& \\
	& A^T \vlam = (\nabla V_\vc.g(\vx))^T \\
	& \vb^T.\vlam \geq -\nabla V_\vc.f(\vx) \,.
\end{array}
\end{equation}
The first constraint is simply a linear constraint. Each of other
conditions will yield a quantifier-free formulae in nonlinear real
arithmetic theory (QF\_NRA) and one can use SMT solvers to solve them quite
efficiently.

\paragraph{Relaxations:}
While SMT solvers can solve such QF\_NRA formulae, they are not super
efficient when the number of variables is large. 

Going further, instead of SMT solvers, one can use other
kind of relaxations. Since we are dealing with polynomial dynamics and
the CLF $V$ is also polynomial, we can use relaxations used for
polynomial optimization problems.
While SOS relaxation has been very
popular, the fact that SOS programming~\cite{prajna2002introducing} 
(And similarly SDSOS programming~\cite{ahmadi2014dsos}) does not provide a 
counter-example encourages us to use its dual 
(LMI relaxation)~\cite{lasserre2001global}.

To be concise, in the LMI relaxation, 
the state space is represented
by a positive semi-definite matrix $Z$ instead of $\vx$. In fact, each
element of $Z$ represents a monomial in $\vx$. More formally,
let $\vz$ be vector ($l = |\vz|$) of monomials in $\vx$ with degree up to $d$. Furthermore, any polynomial $p(\vx)$ with degree up to $2d$ can be written as $\langle P, \vz \vz^T \rangle$, where $P$ is a symmetric $l \times l$ matrix.
$\vz \vz^T$ yields a matrix which is
 \begin{compactenum}
 \item rank 1
 \item positive semi-definite	
 \end{compactenum}
For LMI relaxation, the first constraint is dropped and simply only positive semi-definiteness property is preserved. To achieve this, symmetric matrix $Z$ is introduced. We assume elements of $Z$ are independent. In addition, $Z \succeq 0$. This relaxed $Z$ approximates $\vz \vz^T$ and any polynomial $p(x)$ is relaxed to $\langle P, Z \rangle$. 

\begin{example} \label{ex:lmi}
	Assume $p(\vx) = x_1^2 - 1.5x_1x_2 + x_2^2 + x_1 - 2$. Since degree of $p$ is $2$, we can consider $d = 1$ and $\vz^T = [ 1 \ x_1 \ x_2 ]$. Then a $3 \times 3$ positive semi-definite matrix $Z$ is introduced to approximate $\vz \vz^T$. Since
\begin{align*}
 p(\vx) & = \langle P, \vz \vz^T \rangle \\
	 & = \langle \left[ \begin{array}{ccc}
		-2 & 0.5 & 0 \\
		0.5 & 1 & -0.75 \\
		0 & -0.75 & 1
	\end{array} \right] 
	\left[ \begin{array}{ccc}
		1 & x_1 & x_2 \\
		x_1 & x_1^2 & x_1x_2 \\
		x_2 & x_1x_2 & x_2^2
	\end{array} \right] \rangle \,,
\end{align*}
	in the LMI relaxation, $\langle P, Z \rangle$ represents $p(\vx)$:
\begin{align*}
 \langle P, Z \rangle
	  = \langle \left[ \begin{array}{ccc}
		-2 & 0.5 & 0 \\
		0.5 & 1 & -0.75 \\
		0 & -0.75 & 1
	\end{array} \right] 
	\left[ \begin{array}{ccc}
		1 & z_1 & z_2 \\
		z_1 & z_3 & z_4 \\
		z_2 & z_4 & z_5
	\end{array} \right] \rangle \,.
\end{align*}	
\end{example}

\paragraph{Our Implementation:} While using LMI relaxation may seem 
straightforward, there is a catch.
Changing the structure for the witness space $X$, changes the interface of 
the learning framework. So, witnesses are no longer a vector $\vx$, 
but a positive semi-definite matrix $Z$. One solution is to just project
the witness $Z$ into the $X$. However, this method
simply fails as it can provide a spurious counter-example. In fact, the learner
gets confused, because the counter-example provided by the teacher is
not a valid counter-example. 

As a result, the learner and 
the demonstrator need to change their interface and use $\Z (:\mathbb{S}^+)$
instead of $X$. Notice that the
learner uses polynomials $f$, $g$ and $V$, which can be written as linear 
functions in $Z$, and the learner can
generate linear constraints from a given observation $(Z, \vu)$.

Our verifier implementation uses Gloptipoly~\cite{henrion2009gloptipoly} toolbox. 
Gloptipoly in turn uses Yalmip~\cite{lofberg2004yalmip}, which
is configured to use Mosek~\cite{mosek2010mosek} for the SDP solver.



\subsection{CO-Design:}
These oracles and the learner are part of the framework. While
the discussed method is theoretically complete and it separates these
components through some interfaces, it is essential to keep in mind that
considering all these components beside each other will lead to a
better performance. These issues will also be covered in 
this section.

\paragraph{Verifier and Learner:}
The verifier can provide not only any counter-example, but a good one 
(if one exists) to
improve the learning procedure (faster learning). This technique has 
been investigated before~\cite{jha2015theory,ravanbakhsh2015counter}. 
In our case, finding a good
counter-example is equivalent to adding an objective function to the SDP problem generated by the LMI relaxation.
More precisely, instead of solving for 
$(\exists \vx) \ \mbox{ s.t. } g_i(\vx) \succeq 0$, we solve for
\[
\maximize \gamma \ \mbox{ s.t. } g_i(\vx) \geq \gamma I \,
\]
where $I$ is the identity matrix of proper size. 
If $\gamma^*$ is positive, then there is a counter example and
by maximizing $\gamma$, we provide a counter-example that violates
the constraints severely.


\paragraph{Verifier and Demonstrator:}
Next, we consider a simple technique that the demonstrator
could use when the verifier is using the LMI relaxation. Notice that the demonstrator
should provide $\vu$ for a counter-example $Z$.
The demonstrator can simply project the counter-example $Z^*$ into 
$\vx^*$ and generate the data for $\vx^*$. However, it would be a more 
flexible demonstration if the demonstrator could provide different 
control inputs for different $Z$'s with the
same projection $\vx$. 
One way for accomplishing such goal is to use $Z$
for the first transition in the discretized model used in the MPC scheme. 
More precisely, the constraints used for the MPC optimization can have the 
following form:
\[
\vx(\tau) = \hat{F}(Z, \vu), (\forall t > \tau) \ x(t) = F(\vx(t-\tau), \vu(t-\tau))\,,
\]
where $\hat{F}$ is $F$ written as a function linear in $Z$.

\paragraph{Demonstrator and Learner:}
Recall that learner does not tolerate any error when
learning a concept from training data. Moreover,
the learner ability is restricted to some fixed
template(Eq.~\eqref{eq:clf-template}). Such 
restriction can lead to failure in practice unless
we compensate the learners inflexibility with 
the demonstrator flexibility
(a.k.a coaching~\cite{he2012imitation}). 
The demonstrator can consider the learners ability and 
adjust themselves to achieve better results.

Since we are not concerned
about the optimality of the controller and correctness is the ultimate goal,
we propose to use cost functions as a coaching tool. For example, if we are
interested in quadratic
CLFs, then these cost functions should be quadratic in $\vx$.

Another essential part of coaching is to consider best control input
if many solution exists.
Each input $\vu_i \in \reals$ has its own contribution for decrease 
of $V$ through $(\nabla V.g(\vx^*))_i.\vu_i$. The demonstrator can 
convey these  information to the learner by providing proper $\vu^*$.
The idea is to give a large value to $|\vu_i|$ only if $\vu_i$ is 
critical for stabilization at state $\vx^*$. Otherwise, if $\vu_i$ 
does not have a large contribution in decreasing value of $V$, the 
data generator will reduces $|\vu_i|$. This is in contrast with 
optimality, because if one wishes to decrease $V$ as fast as possible,
the solution would be an input with biggest norm. To achieve such
coaching, we propose to add a $\norm{\vu}^2$ as a penalty to the cost
of the MPC controller. Then, the controller uses large values for
$\vu^*_i$ only if it is necessary.

Recall that we wish $\dot{V} < 0$ by choosing proper
value for $\vu$. The value of $\vu_i$ would decrease 
$\dot{V}$ by $(\nabla V.g(\vx^*))_i.\vu_i$.
Looking from learner perspective, if for $\vx^*$, $|\vu_i|$ is small,
the value of $(\nabla V.g(\vx^*))_i$ can be anything and the observation
does not enforce any restriction on that. 
On the other hand, if for example
$\vu_i >> 0$, then $(\nabla V.g(\vx^*))_i \leq 0$, which adds more
restrictions on $(\nabla V.g(\vx^*))_i$. This way, the teacher hints 
how much each input is essential (not optimal) for a given state $\vx^*$. 
This leads to a more flexible learning process, where only critical 
restrictions will be enforced on $V$.

In summary, we use the following standard cost functions for coaching:

\[
Cost(\vx, \vu) = \vx^T Q \vx + \vu^T R \vu \ , \ \  TCost(\vx) = \frac{T}{\tau} \vx^T Q_F \vx \,.
\]


Putting all these co-design techniques together, our method can practically
solve interesting problems while without co-design, the framework can fail
even for very small and simple problems.




 
